NSFlow: An End-to-End FPGA Framework with Scalable Dataflow Architecture for Neuro-Symbolic AI

Neuro-Symbolic AI (NSAI) is an emerging paradigm that integrates neural networks with symbolic reasoning to enhance the transparency, reasoning capabilities, and data efficiency of AI systems. Recent NSAI systems have gained traction due to their exceptional performance in reasoning tasks and human-AI collaborative scenarios. Despite these algorithmic advancements, executing NSAI tasks on existing hardware (e.g., CPUs, GPUs, TPUs) remains challenging, due to their heterogeneous computing kernels, high memory intensity, and unique memory access patterns. Moreover, current NSAI algorithms exhibit significant variation in operation types and scales, making them incompatible with existing ML accelerators. These challenges highlight the need for a versatile and flexible acceleration framework tailored to NSAI workloads. In this paper, we propose NSFlow, an FPGA-based acceleration framework designed to achieve high efficiency, scalability, and versatility across NSAI systems. NSFlow features a design architecture generator that identifies workload data dependencies and creates optimized dataflow architectures, as well as a reconfigurable array with flexible compute units, re-organizable memory, and mixed-precision capabilities. Evaluating across NSAI workloads, NSFlow achieves 31x speedup over Jetson TX2, more than 2x over GPU, 8x speedup over TPU-like systolic array, and more than 3x over Xilinx DPU. NSFlow also demonstrates enhanced scalability, with only 4x runtime increase when symbolic workloads scale by 150x. To the best of our knowledge, NSFlow is the first framework to enable real-time generalizable NSAI algorithms acceleration, demonstrating a promising solution for next-generation cognitive systems.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Sections/X_Profiling.tex <==
\section{Computational Behavior of NVSA}
\label{sec:profile}

This section characterizes the computational behavior of neurosymbolic AI with NVSA as a case study (Sec.~\ref{subsec:profiling_setup}-\ref{subsec:profiling_memory}), and provides specific insights for computer architects (Sec.~\ref{subsec:opportunity}).

\begin{figure*}[t!]
\centering\includegraphics[width=2.05\columnwidth]{Figs/Profiling/e2e_backend_latency.pdf}
\vspace{-0.1in}
        \caption{\textbf{End-to-end and symbolic latency breakdown.} \textbf{(a)} Benchmark NVSA on Jetson TX2, Xavier NX and RTX GPU, showing that real-time performance cannot be satisfied and symbolic backend is the bottleneck. \textbf{(b)} Benchmark NVSA on various RPM task sizes on RTX GPU, indicating the potential scalability problem and consistent symbolic bottleneck. \textbf{(c)} Benchmark NVSA symbolic on RPM task with various attributes and sizes, illustrating that rule probability computation and VSA-to-PMF steps are bottlenecks within symbolic operations.}
        \label{fig:profiling_latency_e2e}
        \vspace{-5pt}
\end{figure*}

\subsection{Profiling Setup}
\label{subsec:profiling_setup}
To understand the real-device efficiency of neurosymbolic AI workload, we profile our adopted NVSA model~\cite{hersche2023neuro} as elaborated in Sec.~\ref{subsec:nvsa_pipeline}, in terms of runtime and memory footprint for solving RPM cognitive problem on three devices, including RTX 2080Ti GPU (250~W), Xavier NX (20~W), and Jetson TX2 (15~W), respectively.


\subsection{Compute Latency Analysis}
\label{subsec:profiling_latency}

\textbf{End-to-end latency breakdown.}
Fig.~\ref{fig:profiling_latency_e2e}\textcolor{ACMPurple}{a} illustrates the end-to-end latency breakdown of NVSA on RPM cognitive tasks. We can observe that 
(1) the real-time performance cannot be satisfied on all three devices, e.g., RTX 2080Ti GPU takes 380~s and TX2 takes 7507~s for 3$\times$3 RPM task. Even if more computing resources are available to reduce NN inference time, the significant overhead of vector-symbolic-based rule reasoning will still prohibit real-time execution.
(2) Symbolic backend consistently dominates runtime. For example, Step~\circled{4} counts for 87\% of total NVSA inference time on RTX 2080Ti while its floating-point operations (FLOPS) count for only 19\% of total NVSA FLOPS, indicating that the symbolic operations may not be well accelerated by GPU.
(3) Symbolic backend reasoning computation depends on the result of the frontend neuro workload and thus lies on the critical path during inference. 

\textbf{End-to-end latency scalability.} Fig.~\ref{fig:profiling_latency_e2e}\textcolor{ACMPurple}{b} indicates that the neuro vs. symbolic runtime proportion shown remains relatively stable across various task sizes, whereas the total runtime increases quadratically. For example, when the test set size increases from 2$\times$2 to 3$\times$3, the symbolic workload runtime percentage slightly changes from 91.59\% to 87.35\% while the total NVSA runtime increases by 5.02$\times$, indicating the potential scalability bottleneck of neurosymbolic models.

% Neuro perception frontend ratio increases with the problem size scaling; For example, when the test set size increases from 2$\times$2 to 3$\times$3, the symbolic workload runtime percentage only increases from 92.06\% to 94.71\%, but the total runtime of the NVSA model increases by 5.02$\times$, indicating the potential scalability bottleneck of NSAI models.



% \begin{figure}[t!]
% \centering
% \includegraphics[width=\columnwidth]{Figs/Profiling/end_to_end_latency.pdf}
% \vspace{-0.25in}
%         \caption{\textbf{End-to-end latency breakdown.} \textbf{(a)} Benchmark NVSA on Jetson TX2, Xavier NX and RTX GPU, showing that real-time performance cannot be satisfied and symbolic backend is the bottleneck. \textbf{(b)} Benchmark NVSA on various RPM task sizes, showing the potential scalability problem and consistent symbolic bottleneck.  \blue{add label for arrow, perf/W,  EDP, add comparison of GPU and cogsys}}
%         \label{fig:profiling_latency_e2e}
%         \vspace{-5pt}
% \end{figure}

\textbf{Symbolic backend operation analysis.} Inspired by the lucrative bottleneck of the symbolic backend, we analyze the detailed operators of Step \circled{4} (Fig.~\ref{fig:nvsa_backend_operation}). We observe that the rule symbolic reasoning consists of Step \circled{4}-\circledwhite{1} transforming PMF attribute to vector-symbolic representation (vector-matrix multiplication), Step \circled{4}-\circledwhite{2} rule probabilistic computation (circular convolution as Eq.~\ref{eq:cir_conv}) and Step \circled{4}-\circledwhite{3} transforming vector-symbolic representation to PMF (vector-vector multiplication), where the inter-step operations are sequential. 

% Fig.~\ref{fig:nvsa_backend_operation} dissects the symbolic backend operation.
% Observations: 
% (1) S1 vector-matrix multiplication;
% (2) S2 circular convolution;
% (3) S3 vector-vector multiplication.

\begin{figure}[t!]
\vspace{-3pt}
\includegraphics[width=\columnwidth]{Figs/Algorithm/nvsa_backend_ops.pdf}
        \caption{\textbf{NVSA Symbolic backend operation.} Symbolic backend consists of three steps with high-dimensional vector-matrix multiplication, circular convolution, vector-vector multiplication.}
        \label{fig:nvsa_backend_operation}
        \vspace{-12pt}
\end{figure}

\textbf{Symbolic backend latency breakdown.} 
Fig.~\ref{fig:profiling_latency_e2e}\textcolor{ACMPurple}{c} demonstrates the latency breakdown of reasoning backend Step \circled{4} on RTX 2080Ti GPU for five attributes and three constellations of RPM cognitive problem. We can observe that (1) Step \circled{4}-\circledwhite{2} and Step \circled{4}-\circledwhite{3} consistently dominates the runtime. The reason is Step \circled{4}-\circledwhite{1} PMF-to-VSA transformation is shared with all rules while the Step \circled{4}-\circledwhite{2} probabilistic reasoning and Step \circled{4}-\circledwhite{3} VSA-to-PMF processes run sequentially and separately for each underlying rule. (2) Both \circled{4}-\circledwhite{2} and \circled{4}-\circledwhite{3} operate on $d$=1024 vectors, while \circled{4}-\circledwhite{2} exhibits higher latency, indicating that circular convolution may not be well supported by GPUs. (3) In neurosymbolic systems, the element-wise operations stemming from high-dimensional distributed vector computations for symbolic reasoning representation are difficult to process efficiently on GPUs. Therefore, the challenges of accelerating these computations will become increasingly important as the task and feature complexities further grow.

% Fig.~\ref{fig:backend_runtime_gpu} shows the execution time in percentage for different attributes on Titan RTX (TU102) GPU. The breakdown is shown for center single(1x1), distribute four(2x2) and distribute three(3x3) configurations. The number and position attributes come in picture for distribute four and distribute nine configurations while type, size and color attributes apply to all configurations.
% Observations: 
% (1) S2 and S3 dominate the latency over S1. One of the reasons is that S1 is common for all of the rules while S2 and S3 are executed sequentially for each rule. S1 is vector multiplication between pmf vector of size n (attribute dimension) and binary sparse codebook matrix of size m x attribute dimension. M is fixed by algorithm \cite{hersche2023neuro} as 1024 and attribute dimension is 8 for number, 5 for type, 10 for color, 6 for size and 511 for position. Since position has the largest attribute dimension, percentage of S1 execution time is highest as can be seen from the graph. 

% (2) Both S2 and S3 operate on vectors of length 1024. S2 has a slightly higher latency than S3 for most cases. It is because circular convolution operation takes more time than vector-vector multiplication for the same input dimensions. 
% (5) why GPU is not efficient: Notably, the element-wise operations usually stem from high-dimensional distributed vector computations (e.g., binding, bundling, and permutation) for symbolic representation, which is difficult to process efficiently on GPUs.
% predominately due to the sequential and computational-intensive rule detection during the involved reasoning procedure
% Therefore, the challenges of accelerating these computations will become increasingly important as the task and feature complexities further grow.

% Fig.~\ref{fig:prolifing_latency_backend} shows the execution time for different attributes in center single configuration of Raven dataset. It can be inferred that S2 (circular convolution) and S3 (vector-vector multiplication) have much larger execution time than S1 (vector-matrix multiplication). One of the reasons is that S1 can be executed once while S2 and S3 are to be executed sequentially for each rule.

% \begin{figure}[t!]
% \includegraphics[width=\columnwidth]{Figs/Profiling/backend_latency.pdf}
% \vspace{-0.2in}
%         \caption{\textbf{Symbolic backend latency breakdown.} Benchmark NVSA symbolic backend on RPM task with various attributes and sizes, illustrating that the rule probability computation and VSA-to-PMF transformation steps are bottlenecks. \blue{combine three subplots with fig.3}}
% \label{fig:backend_runtime_gpu}
%         \vspace{-5pt}
% \end{figure}

\subsection{Memory Requirement Analysis}
\label{subsec:profiling_memory}

\textbf{Memory footprint.}
Fig.~\ref{fig:e2e_memory} characterizes the memory footprint for end-to-end NVSA workload. We can observe that Step \circled{1} neuro frontend and Step \circled{2} codebook accounts for >90\% memory footprint. This is because NVSA frontend enables the expression of many more object combinations than vector space dimensions, requiring $\boldsymbol{W}$ to be large enough to contain all object combinations and ensure quasi-orthogonality. It is worth noting that by leveraging probabilistic abduction reasoning in Steps \circled{3}-\circled{5}, NVSA alleviates the symbolic operation memory requirement compared to exhaustive search.

% The NVSA symbolic reasoning is 
% Observation: (1) resnet and codebook takes lot of memory thus we optimize them through quantization and factorization; (2) symbolic operation require less than large search, making them competitive;

% Add plot: memory requirement for each stage, serve as another motivation for HW/SW optimization.
\textbf{Communication bandwidth.} The symbolic backend requires streaming vector elements to circular convolution computing units, increasing the memory bandwidth pressure. Optimizing the compute dataflow and leveraging the scalable and reconfigurable processing element can help provide this bandwidth, as we will demonstrate via CogSys.

% mention data dependency (parallel/sequential computation), operator size

% ToDo: memory usage/access pattern, roofline analysis (compute-bound / memory bound), communication bandwidth analysis

% \subsection{Sparsity Analysis}
% \label{subsec:profiling_sparsity}

% Fig.~\ref{fig:profiling_sparsity_S1}, Fig.~\ref{fig:profiling_sparsity_S2_dist3}, and Fig.~\ref{fig:profiling_sparsity_S2} analyze the sparsity of NVSA symbolic reasoning backend.
% Observations:
% (1) Sparsity ratio is high ($>$95\%);
% (2) Sparsity has variations for some attributes;
% (3) Unstructured sparsity.

% \begin{figure}
%      \centering
%      \includegraphics[width=0.45\textwidth]{Figs/s1_sparsity.pdf}
%      \caption{Breakdown of s1 sparsity for different attributes}
%      \label{fig:profiling_sparsity_S1}
%      \vspace{-5pt}
% \end{figure}

% \begin{figure}
%      \centering
%      \includegraphics[width=0.45\textwidth]{Figs/s2_sparsity_distribute_three.pdf}
%      \caption{Breakdown of s2 sparsity for the distribute three rule for different attributes}
%      \label{fig:profiling_sparsity_S2_dist3}
%      \vspace{-5pt}
% \end{figure}

% \begin{figure}
%      \centering
%      \includegraphics[width=0.45\textwidth]{Figs/s2_sparsity_rest.pdf}
%      \caption{Breakdown of s2 sparsity for rest of the rules for different attributes}
%      \label{fig:profiling_sparsity_S2}
%      \vspace{-5pt}
% \end{figure}

\subsection{Identified Opportunities for Optimization}
\label{subsec:opportunity}
\textbf{Memory optimization for codebook.} Given the quasi-orthogonality of the representations in Step \circled{2} codebook $\boldsymbol{W}$ and its large memory footprint, we hypothesize that substituting $\boldsymbol{W}$ with a set of smaller codebooks by potentially exploiting a dynamical system based on vector-symbolic operators can reduce on-chip memory requirement while maintaining its reasoning accuracy (Sec.~\ref{subsec:algo_factorzation}). 
% It is highly desirable to develop techniques that can efficiently factorize product vectors 

\textbf{Compute unit optimization for circular convolution.} Step \circled{4} symbolic reasoning operations are the bottleneck of cognitive tasks, it is thus highly desirable to develop customized and reconfigurable processing elements to efficiently support single and multiple circular convolutions (Sec.~\ref{subsec:hw_circular_conv}). 

\textbf{Runtime optimization for dynamic scheduling.} The sequential operations of inter-Steps \circled{1}-\circled{5} and intra-Steps \circled{4}-\circledwhite{1} to \circled{4}-\circledwhite{3} burden the NVSA end-to-end runtime, so we hypothesize that dynamically scheduling the different steps with inter- and inter-step parallelism and domain-specific dataflow can reduce the overall latency (Sec.~\ref{subsec:algo_parallel} and Sec.~\ref{subsec:scheduling}).

\textbf{Scalability optimization for complex cognitive task.} The total NVSA runtime quadratically increases with problem size and attributes increasing, it is thus highly desirable to develop scalable architecture to support future complex cognitive tasks towards explainable and trustworthy systems (Sec.~\ref{subsec:folding} and Sec.~\ref{subsec:hardware_systolic_array}).
% latency analysis $\rightarrow$ optimize circular conv

% latency analysis $\rightarrow$ scheduling scheme

% latency and bandwidth analysis $\rightarrow$ better scalability with scaleup and scaleout and sara-like arch

% memory analysis $\rightarrow$ quantization and factorization to reduce size of step 1/2.
Inspired by the above workload characterizations and optimization opportunities, we propose CogSys, an algorithm-hardware co-design framework dedicated to neurosymbolic AI acceleration, aiming to win both reasoning efficiency and cognition capability in NVSA systems.

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{Figs/Profiling/end_to_end_memory.pdf}
\vspace{-0.2in}
        \caption{\textbf{Memory footprint analysis.} The neuro and codebook frontends are memory bottlenecks and account for >90\% of storage. Our proposed \NAME  compresses overall storage by 4.75$\times$.}
\label{fig:e2e_memory}
        \vspace{-5pt}
\end{figure}
% \begin{itemize}
%     \item Parallelism: patch-level parallelism (PLP) and attribute-level parallelism (ALP).
%     \item Intra-Stage Dataflow: Optimized compute unit to support high-dimensional circular conv, VMM, VVM, etc computations.
%     \item Inter-Stage Dataflow: S1/S2/S3 reconfigurability / pipelining.
% \end{itemize}

% \begin{itemize}
%     \item Latency and memory profiling of various neurosymbolic AI workloads. 
%     \begin{itemize}
%         \item CPU and GPU (high-end and embedded), root cause why they are inefficient.
%         \item Cache on-chip memory size.
%         \item Communication bandwidth. Roofline analysis.
%         \item Sparsity of high-dimensional vectors.
%         \item We use neuro-vector-symbolic architecture (NVSA) to drive the system architecture in this work, though it can be extended to work with other neurosymbolic algorithms as well. 
%         \item Why NVSA: show its advantages in superior accuracy in human-level cognitive reasoning tasks, but with low speed and high energy.
%     \end{itemize}
%     \item Operation graph analysis. 
%     \begin{itemize}
%         \item Algorithm flow and identify concurrent/sequential processing, if has dependencies. 
%         \item NVSA exposes panel-level parallelism (PLP) and rule-level parallelism (RLP), data reuse, and other dataflow opportunities. Provide architects with insights on designing efficient systems for running neurosymbolic algorithms. 
%         \item Identify the size of operators.
%     \end{itemize}
%     \item Motivate the simulator and hardware design from profiling.
%     \begin{itemize}
%         \item If we can reduce the energy consumption of the compute ops by implementing them in hardware, pack a lot of compute engines in a small form factor, we can advance the cognitive AI in mobile autonomous agents.
%     \end{itemize}
% \end{itemize}

% \counterwithin{figure}{section}
% \captionsetup[figure]{labelsep=period, name=Figure}
% \renewcommand\thefigure{\thesection.\arabic{figure}}

% Many NSAI models and algorithms have been developed for various tasks in recent years. In this section, we will use NVSA as a main example, to discuss their structure, performance and profiling results.
 
% \subsection{NVSA algorithm}

% NVSA is one of the state-of-the-art algorithms combining neural networks and symbolic AI approaches to solve RPM task. In order to remedy the inability of current neural networks to recover distinct objects from their joint representations, it integrates VSA (Vector-Symbolic Architecture) for its symbolic representation, which also performs as a bridge between the Neural Network at the frontend and the symbolic reasoning part at the backend thanks to its HDC (High-Dimensional Computing) features. The model is able to achieve XX accuracy on I-RAVEN task set, even exceeding human performance blahblah... 

% In this section we will discuss NVSA algorithm operations and its profiling results. 

% \begin{comment}
% %Hanchen
% figure3.1
% \item x8 => xN
% \item split rule detector

% figure 3.2
% \item show more result: 2x2, centered, different rules/attributes

% \item Algorithm optimization
% read/write?
% locality?

% \item memory optimization
% \end{comment}

% \subsubsection{NVSA Frontend}
% \subsubsection{NVSA Backend}




==> Sections/X_Related_Work.tex <==
% \vspace{-5pt}
\section{Related Works}
\label{sec:related}
 
\subsection{Neurosymbolic AI Workloads}
\label{subsec:related_nsai}
Neurosymbolic AI represents an interdisciplinary approach that synergistically combines symbolic reasoning with neuro learning to create intelligent systems.
% leveraging complementary strengths to enhance the performance and interpretability of the models. 
Neurosymbolic AI holds significant potential for enhancing explainability, robustness, and trustworthiness of next-generation cognitive applications including collaborative robotics, mixed-reality, and human-AI interactions. AI agents can reason and make decisions in a robust and explainable manner, and intelligence is pervasively embedded and untethered from the cloud.
Based on how neuro and symbolic components integrate into a cohesive system, neurosymbolic AI can be categorized into three groups, i.e., Symbolic[Neuro], Neuro[Symbolic], and Neuro$|$Symbolic. Symbolic[Neuro]~\cite{zhang2020alphazero} empowers symbolic reasoning with the statistical learning capabilities of NNs, and Neuro[Symbolic]~\cite{badreddine2022logic,hohenecker2020ontology,dongneural} empowers NNs with the explainability and robustness of symbolic reasoning.
Neuro$|$Symbolic~\cite{hersche2023neuro,pryor2022neupsl,manhaeve2021neural,yang2020neurasp,yi2020clevrer} combines NN and symbolic systems in a pipeline, where each specializes in complementary tasks. \emph{Neuro$|$Symbolic attracts most algorithmetic developments and achieves SOTA reasoning performance, thus \NAME co-design framework targets this category and envisions it to be adaptive to future neurosymbolic workloads.}
% targets and is adaptable to future neurosymbolic workloads.
% Neurosymbolic AI promises many possibilities for AI systems that acquire human-like communication and reasoning capabilities, enabling them to recognize, classify, and adapt to new situations autonomously.


\vspace{-5pt}
\subsection{Accelerators for Emerging Applications}
\label{subsec:related_accelerator}
Over the past years, computer architects both from academia and industry have proposed a vast array of custom architectures, most notably for accelerating machine learning, specifically DNN training and inference across a variety of use cases ranging from edge \cite{genesys, zhou2022ml, tambe202216} to large scale cloud systems \cite{tpuv4, simba, rapid, brainwave}.
In addition, hardware acceleration has been found to useful in other applications like genome sequencing \cite{fujiki2020seedex, fujiki2018genax}, line rate processing in cloud use cases \cite{swamy2022taurus, firestone2018azure}, in vision pipeline of mobile processors\cite{zhu2018euphrates, liu2022s2ta, liu2020systolic}, encoding-decoding of video library content on cloud \cite{ranganathan2021warehouse} etc. Most recently hardware acceleration is emerging as \textit{the} enabler for secure  execution using end-to-end fully homomorphic execution\cite{f1, samardzic2022craterlake, geelen2022basalisc, nabeel2023cofhee}. 
With the slowdown of benefits of device scaling in the recent years, custom architecture design is a pragmatic approach to ensure simultaneous improvements in performance and efficiency.  
%
\textit{Despite the presence of large body of work in accelerator design for applications, \NAME is the first proposal to enable efficient execution of NVSA and neurosymbolic algorithms in general.}

==> Tables/algo_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
% \scriptsize
\centering
\caption{\textbf{\NAME Algorithm Optimization Performance.} \textnormal{\NAME exhibits comparable reasoning capability with the proposed quantization. Neurosymbolic achieves higher cognitive accuracy than neuro-only methods.}}
% \vspace{0.05in}
\renewcommand*{\arraystretch}{1.3}
\setlength\tabcolsep{2.1pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|ccc|cc|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dataset\\ Accuracy\end{tabular}} & \multicolumn{3}{c|}{Neurosymbolic Model in \NAME}                                                                                      & \multicolumn{2}{c|}{Non-neurosymbolic}        & \multirow{2}{*}{Human} \\ \cline{2-6}
    & \multicolumn{1}{c|}{NVSA (FP32)} & \multicolumn{1}{c|}{NVSA (INT8)} & \begin{tabular}[c]{@{}c@{}}NVSA-MP\\ (INT8 for NN, \\ INT4 for Symb)\end{tabular} & \multicolumn{1}{c|}{ResNet18}   & GPT-4       &                        \\ \hline
RAVEN                                                                       & \multicolumn{1}{c|}{98.9\%}      & \multicolumn{1}{c|}{98.7\%}    & ?\%                                                                               & \multicolumn{1}{c|}{53.4\%}     & 89.0\%      & 84.4\%                 \\ \hline
I-RAVEN                                                                     & \multicolumn{1}{c|}{99.0\%}      & \multicolumn{1}{c|}{98.8\%}    & ?\%                                                                               & \multicolumn{1}{c|}{40.3\%}     & 86.0\%      & 78.6\%                 \\ \hline
PGM                                                                         & \multicolumn{1}{c|}{68.7\%}      & \multicolumn{1}{c|}{68.4\%}    & ?\%                                                                               & \multicolumn{1}{c|}{36.8\%}     & 56.0\%      & N/A                    \\ \hline
Memory                                                                & \multicolumn{1}{c|}{32MB}  & \multicolumn{1}{c|}{8MB} & 5.5MB                                                                       & \multicolumn{1}{c|}{42MB} & 1.7TB & N/A                    \\ \hline
\end{tabular}
}
\label{tab:eval_acc}
% \vspace{-5pt}
\end{table}


==> Tables/deployment.tex <==
\begin{table*}[t!]
\vspace{-0.15in}
\centering
\caption{\textbf{Design Configuration and FPGA deployment.}}
% \Huge
\small
\renewcommand*{\arraystretch}{1.0}
% \setlength\tabcolsep{2pt}
\resizebox{\linewidth}{!}{%
\centering
\setlength\tabcolsep{5pt}

\begin{tabular}{|cl|cc|cc|c|ccc|c|cccccc|c|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Workloads}} & \multicolumn{2}{c|}{Precision}   & \multicolumn{2}{c|}{AdArray Configuration}                                                                                                                                & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SIMD \\ Size\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}On-chip \\ SRAM Blocks \\ (BRAM)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}On-chip \\ Cache \\ (URAM)\end{tabular}} & \multicolumn{6}{c|}{ZCU-104 Utilization}                                                                                                           & \multirow{2}{*}{Frequency} \\ \cline{3-6} \cline{8-10} \cline{12-17}
\multicolumn{2}{|c|}{}                           & \multicolumn{1}{c|}{Neural}   & Symb & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Size \\ (H, W, N)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Default Partition \\ ($\bar{N}_l$ : $\bar{N}_v$)\end{tabular} &                                                                       & \multicolumn{1}{c|}{MemA1, MemA2}          & \multicolumn{1}{c|}{Mem B}        & Mem C        &                                                                                     & \multicolumn{1}{c|}{DSP}  & \multicolumn{1}{c|}{LUT}  & \multicolumn{1}{c|}{FF}   & \multicolumn{1}{c|}{BRAM} & \multicolumn{1}{c|}{URAM} & LUTRAM &                            \\ \hline
\multicolumn{2}{|c|}{NVSA}                       & \multicolumn{1}{c|}{INT8} & INT4 & \multicolumn{1}{c|}{16, 16, 8}                                                 & 7 : 1                                                                                    & 32                                                                    & \multicolumn{1}{c|}{2.7 MB, 1.1 MB}        & \multicolumn{1}{c|}{2.7 MB}       & 1.6 MB       & 16.2 MB                                                                             & \multicolumn{1}{c|}{93\%} & \multicolumn{1}{c|}{56\%} & \multicolumn{1}{c|}{43\%} & \multicolumn{1}{c|}{73\%} & \multicolumn{1}{c|}{62\%} & 24\%   & 100 MHz                    \\ \hline
\multicolumn{2}{|c|}{MIMONet}                    & \multicolumn{1}{c|}{INT8} & INT8 & \multicolumn{1}{c|}{32, 16, 4}                                                 & 3 : 1                                                                                    & 32                                                                    & \multicolumn{1}{c|}{3.4 MB, 1.2 MB}        & \multicolumn{1}{c|}{3.4 MB}       & 2.1 MB       & 20.1 MB                                                                             & \multicolumn{1}{c|}{93\%} & \multicolumn{1}{c|}{48\%} & \multicolumn{1}{c|}{38\%} & \multicolumn{1}{c|}{91\%} & \multicolumn{1}{c|}{74\%} & 20\%   & 100 MHz                    \\ \hline
\multicolumn{2}{|c|}{LVRF}                       & \multicolumn{1}{c|}{INT8} & INT4 & \multicolumn{1}{c|}{16, 16, 8}                                                 & 7 : 1                                                                                    & 32                                                                    & \multicolumn{1}{c|}{2.7 MB, 0.96 MB}       & \multicolumn{1}{c|}{2.7 MB}       & 1.4 MB       & 15.5 MB                                                                             & \multicolumn{1}{c|}{93\%} & \multicolumn{1}{c|}{56\%} & \multicolumn{1}{c|}{43\%} & \multicolumn{1}{c|}{71\%} & \multicolumn{1}{c|}{58\%} & 24\%   & 100 MHz                    \\ \hline
\end{tabular}
}

\label{tab:deployment}
\vspace{-15pt}
\end{table*}
